BlinkML: Efficient Maximum Likelihood Estimation with Probabilistic Guarantees

The rising volume of datasets has made training machine learning (ML) models a major computational cost in the enterprise. Given the iterative nature of model and parameter tuning, many analysts use a small sample of their entire data during their initial stage of analysis to make quick decisions (e.g., what features or hyperparameters to use) and use the entire dataset only in later stages (i.e., when they have converged to a specific model). This sampling, however, is performed in an ad-hoc fashion. Most practitioners cannot precisely capture the effect of sampling on the quality of their model, and eventually on their decision-making process during the tuning phase. Moreover, without systematic support for sampling operators, many optimizations and reuse opportunities are lost. In this paper, we introduce BlinkML, a system for fast, quality-guaranteed ML training. BlinkML allows users to make error-computation tradeoffs: instead of training a model on their full data (i.e., full model), BlinkML can quickly train an approximate model with quality guarantees using a sample. The quality guarantees ensure that, with high probability, the approximate model makes the same predictions as the full model. BlinkML currently supports any ML model that relies on maximum likelihood estimation (MLE), which includes Generalized Linear Models (e.g., linear regression, logistic regression, max entropy classifier, Poisson regression) as well as PPCA (Probabilistic Principal Component Analysis). Our experiments show that BlinkML can speed up the training of large-scale ML tasks by 6.26x-629x while guaranteeing the same predictions, with 95% probability, as the full model.

==> additional_exp.tex <==
\section{Additional Experiments}
\label{sec:add:exp}

\input{figures/fig_hyperparam}

\input{figures/fig_exp_model_complexity}


\subsection{Hyperparameter Optimization}

\tofix{
This section studies \system's benefits in hyperparameter optimization.
Specifically, we compared the accuracies of the models (with different feature sets and hyperparameters) trained by \system and a regular system.
As performed by Random Search~\cite{bergstra2011algorithms},
we first generated a sequence of (pairs of) a randomly chosen feature set and a regularization coefficient.
Then, we let \system train a series of 95\% accurate models using the feature set and the regularization coefficient in the sequence.
Similarly, we let the regular system train a series of exact models using the same combination of the feature set and the regularization coefficient.

\cref{fig:exp:hyperparam} shows the result. Each dot in the figure represents a model. In half an hour, \system trained 961 models while the regular system trained only 3 models.
\system found the second-best model (with test accuracy 74\%; found at iteration \#2) in 1.03 seconds, while the regular system took 817 seconds until it trains the second-best model. In 387 seconds, \system found the best model (with test accuracy 75\%; found at iteration \#91).
The sizes of the samples used by \system varied between 10,000 and 9,211,426, depending on the feature set and the regularization coefficient. Note that this is an expected behavior since \system automatically chooses the sample size that is large enough to produce an accurate model. We study this behavior more systematically in the following section.
}


\subsection{Impact of Model Complexity on Estimated Sample Sizes}
\label{sec:exp:model}

\tofix{
We also studied the impact of model complexity on \system's estimated sample size.
Intuitively, if a model is more complex, a larger sample would be needed for training an accurate model (i.e., the model highly similar to the full model). To control the complexity of a model, we varied the regularization coefficient and the number of parameters (i.e., the number of features) of the model. We used LR for this experiment.

\cref{fig:exp:model} shows the results.
On the left (\cref{fig:exp:model:a}), we can see that as the model became less complex (or more rigid with a larger regularization coefficient), the estimated sample size decreased.
On the right (\cref{fig:exp:model:b}), we can see that as the model became more complex (with a larger number of parameters), the estimated sample size increased.
These results demonstrate the adaptive nature of \cref{thm:param_dist}, which \system relies on for estimating sample sizes.
}


==> additional_experiment.tex <==
% \input{exp_statistics}

==> archi.tex <==
%!TEX root = approx_ml.tex



\input{figures/tab_models}


\section{Workflow and Architecture}
\label{sec:archi}

This section describes the internal components of \system and how they operate together to produce an accuracy-guaranteed approximate model.
As depicted in \cref{fig:archi}, \system has four main components: (1) Model Trainer, (2) Model Accuracy Estimator, (3) Sample Size Estimator, and (4) Coordinator.
 Those components are designed to be agnostic to the individual model, using an abstraction introduced in \cref{sec:model:abstract}.
 We then describe the operations of each component in \cref{sec:components}
 and our sampling process in   \cref{sec:sampling}.

% \input{figures/fig_workflow_a}


\input{workflow}




% The , which we denote by , \barzan{why v? why not use the diff itself?}
% computes the difference between two models $m_1(\cdot)$ and $m_2(\cdot)$.


% These ML models include Generalized Linear Models (e.g., linear regression, logistic regression, maximum entropy classifier, Poisson regression) and Probabilistic Principal Component Analysis (PPCA).

% We describe in \cref{sec:accuracy} how \system exploits the characteristics of the above expression for computing the accuracies (i.e., $\varepsilon$) of approximate models.
% Important characteristics of these models are that they include model parameters, and that the values of those model parameters are obtained by finding $\theta$ that satisfies the following expression:
% \begin{equation}
% g_n(\theta) = \nabla f_n(\theta)
% = \left[ \frac{1}{n} \sum_{i=1}^n q(\theta; \xx_i, t_i) \right] + r(\theta)
% = \bm{0}
% \label{eq:support:grad}
% \end{equation}

% However, the users of \system are not required to understand any details (e.g., statistical properties) of these models. Training and making predictions with an approximate model can be accomplished by writing a short piece of code, as in \cref{fig:code}.




% We first present an abstract form that encapsulates the ML models supported by \system. Then, we illustrate with concrete examples how actual ML models, such as logistic regression and PPCA, can be cast into that abstract form.





\ifsubmit
% \vspace{2mm}
\else
\fi

\ignore{
\subsection{Architecture}
\label{sec:components}

% \system's components rely on the abstract form
% \barzan{u re using this `abstract form' in a really scary way. making the reviewer think we don't understand what an abstraction means.}
% presented in \cref{sec:model:abstract}. To exploit the mathematical abstraction in actual ML training, \system defines a class
% \barzan{what does `BlinkML defines a class' even mean?? Is BlinkML a system? if it is then ur sentence makes no sense. if it is a library, then need to say something like
% BlinkML requires the programmer to instantiate an instance of a virtual class called blah ... where threy need to implemnt blah }
% called \emph{model class specification}. In this section, we first define the model class specification and then
% \tofix{Jingyi: Should be depicted or described?}

As depicted in \cref{fig:archi}, \system is comprised of four major components.
We discussed the Coordinator's role in \cref{sec:workflow}. Here, we discuss the remaining components:
Model Trainer, Model Accuracy Estimator, and Sample Size Estimator.




\ph{Model Trainer}
Model Trainer trains a model by finding its optimal parameter value, $\theta$. Model Trainer takes two inputs: (1) a subset $D_n$ of the training set $D$, where $n \le N$, and (2) a model class specification (MCS).

To train and output a model $m_n$, Model Trainer takes a different approach depending on
the size of $D_n$ and
 the given model class specification, as follows.

\li{1. Closed-Form}
% \item \textbf{Closed-form:}
If the MCS includes the optional \texttt{\textbf{solve}} function, Model Trainer simply relies on its \texttt{\textbf{solve}} function to find its optimal model parameters.

\input{figures/fig_trainer_internals}

\li{2. Iterative}
% \item \textbf{Iterative:}
If the \texttt{\textbf{solve}} function is not present, \system uses the \texttt{\textbf{grads}} function and the optimization libraries in the SciPy's \texttt{optimize} module~\cite{scikit-learn}.
To find the optimal parameter values,
 most optimization libraries
 require the gradient $\nabla f_n(\theta)$ of the objective function $f_n(\theta)$.\footnote{The gradient of a function can be numerically approximated using the function itself; however,
these approximations are much slower.}
The gradient is computed by averaging the outputs of the \texttt{\textbf{grads}} function.
% \end{enumerate}
When using SciPy's \texttt{\textbf{optimize}} module,
computing the gradients is typically
 the dominant cost.
Model Trainer therefore computes the \texttt{\textbf{grads}} function either locally or in a distributed fashion, as described next.
(This is depicted in \cref{fig:trainer}.)
% \tofix{Depending on the size of $D_n$, Model Trainer performs either local training with NumPy/SciPy or distributed training with Spark, as described below.}

\li{2.1. Iterative (Local)}
For small- and medium-scale problems ($n <$ 1M, by default),
 the \texttt{\textbf{grads}} function is computed locally
using NumPy (for dense features) or SciPy (for sparse features).


\li{2.2. Iterative (Distributed)}
For large-scale problems ($n \ge$ 1M, by default), \system computes the gradients using multiple workers (via Apache Spark \cite{spark}).
% \yongjoo{It just means distributed computing, which is a known word.} using Spark \cite{spark}.
% When distributing training examples to
% \barzan{did u mean `between'?} \yongjoo{It is from master to workers.}
 % multiple workers, \system \tofix{sets a group of 10,000 training examples as a single element}
To distribute $D_n$ between the remote workers, \system packs each 10K training examples into a single element
of Spark's RDD.
Then, the \texttt{\textbf{grads}} function is invoked on each element of the RDD.
According to our empirical studies, this enables Spark to exploit NumPy's highly-efficient matrix operations for each RDD element.
Note that this distributed computation is possible only because the gradient expression in \cref{eq:abstract:model} has a special structure that enables data-parallelism.
  That is, given $\theta$, $q(\theta; \xx_i, t_i)$ is independent of $q(\theta; \xx_j, t_j)$ for $i \ne j$.

% \tofix{In contrast, when a single training example is set to an element of Spark's RDD, the performance of Spark's native parallelization was worse than NumPy (and even worse than fully local processing).
% This is because the native parallelism is not aware that the operations performed on the elements of RDD are linear algebra operations. Thus, Spark does not exploit fast matrix computations provided by BLAS and ATLAS (which are supported by NumPy and SciPy). Note that this distribution style is only available, since the gradient expressions of the \system-supported  ML models have the special structure that easily enables data-parallelism. That is, $q(\theta; \xx_i, t_i)$ is independent of $q(\theta; \xx_j, t_j)$ given $\theta$ if $i \ne j$.}\barzan{very bad and confusing english. very surprised Morgan hasn't fixed this. please rewrite this heavily}

\vspace{2mm}

The output of Model Trainer is the model $m_n(\cdot) = m({}\cdot{}; \theta_n)$, which includes the parameter $\theta_n$ trained on $D_n$.
\cref{fig:trainer} depicts Model Trainer's input and output.


% Initially, we set each $\xx_i$ as an element of Spark's RDD and let Spark invoke the \texttt{grads} function for every $\xx_i$. However, we found this approach inefficient because  are not exploited.\footnote{NumPy invokes C code, which is typically faster than Java.} As a result, the distributed computations were even slower than the single-node gradient computations that solely relied on NumPy and SciPy. However, when we distributed the feature vectors in a batch mode by setting a list of 10,000 feature vectors as an element of RDD, distributed gradient computations were faster than using a single worker. Thus, \system uses the second approach.


\ph{Model Accuracy Estimator}
Given an approximate model $m_n$,   a confidence level
$\delta$, and an MCS,
Model Accuracy Estimator computes $\varepsilon_n$, such that $v(m_n, m_N) \le \varepsilon_n$ with probability at least $1 - \delta$.

% The second operations is that given a trained model $m_n$ and an approximation contract function $v(m_1, m_2; \varepsilon)$, it estimates the minimum sample size $n'$ such that $\pr(v(m_{n'}, m_N; \varepsilon) = 1) \ge 1 - \delta$, where $m_{n'}$ is an approximate model trained on a simple random sample of size $n'$.

To achieve this goal, Model Accuracy Estimator exploits the fact that both $m_n$ and $m_N$ are essentially the same function (i.e., $m(\cdot)$) but with different model parameters
(i.e., $\theta_n$ and $\theta_N$).
Although we cannot compute the exact value of $\theta_N$ without training the full model $m_N$,
	we can still estimate its probability distribution (we explain this in \cref{sec:accuracy:param}).
Model Accuracy Estimator uses this estimated probability distribution to estimate $m_N$'s probability distribution (or more accurately, the probability distribution of the output of $m_N(\cdot)$).
The probability distribution of $m_N$ is then used to estimate the distribution of $v(m_n, m_N)$, which is the quantity we aim to upper bound. The upper bound $\varepsilon_n$ is determined by
	simply finding the value that is larger than $v(m_n, m_N)$ with probability at least $1-\delta$.
% We describe more details of Model Accuracy Assessor in \cref{sec:accuracy}.
We discuss this process more formally in \cref{sec:accuracy}.

% We also discuss in \cref{sec:confidence:predict} why \system do not employ other more sophisticated alternatives.

% To perform the second operation---estimating $n'$ such that $\pr(v(m_{n'}, m_N; \varepsilon) = 1) \ge 1 - \delta$,


\ph{Sample Size Estimator}
Given an error bound $\varepsilon$, a confidence $\delta$, and the initial model $m_0$, Sample Size Estimator estimates the minimum sample size
 $n'$, such that $v(m_{n'}, m_N) \le \varepsilon$ with probability at least $1 - \delta$.
 Here, $m_{n'}$ is the approximate model trained on a sample of size $n'$, say $D_{n'}$.
The core function of Sample Size Estimator is to compute $\pr(v(m_{n''}, m_N)\allowbreak \le \varepsilon)$ for an arbitrary $n''$.
Note that $v(m_{n''}, m_N)$ is a random variable since its output relies on a random sample $D_{n''}$.
% \tofix{The probability is placed on $v(m_{n''}, m_N)$, since it is a random variable; $D_{n''}$, on which , is a random sample.}

Similar to Model Accuracy Estimator, Sample Size Estimator   exploits the probability distributions of $m_{n''}$ and $m_N$ to compute $\pr(v(m_{n''}, m_N) \allowbreak \le \varepsilon)$.
In this case, however, the model parameters of both $m_{n''}$ and $m_N$ are unknown. Thus, Sample Size Estimator treats both model parameters as random variables and uses the joint probability distribution of $(\hat{\theta}_{n''}, \hat{\theta}_N)$ to estimate $v(m_{n''}, m_N)$,
 where $\hat{\theta}_{n''}$ is the random variable for the unknown model parameter $\theta_{n''}$ of $m_{n''}$.
We describe this process in more details in \cref{sec:sample}.


% How to i.i.d.-sample from the joint probability distribution is presented in \cref{sec:sample:search}.

% An important sub-component of Sample Size Estimator is the module that computes $\pr(v(m_{n''}, m_N) \le \varepsilon)$ for an arbitrary $n''$. The randomness of this expression, $v(m_{n''}, m_N)\allowbreak \le \varepsilon$, stems from that $D_{n'}$ is a random sample.



% Sample Size Estimator finds the minimum sample size $n'$ by performing binary search relying on that $\pr(v(m_{n''}, m_N) \le \varepsilon)$ is a monotonically increasing function of $n''$ in general (since the approximate model $m_{n''}$ becomes closer to the full model $m_N$ as $n'' \rightarrow N$).

% Like Model Accuracy Assessor, the sub-component of Sample Size Estimator also exploits the probability distributions of $m_{n''}$ and $m_N$ for estimating $\pr(v(m_{n''}, m_N) \allowbreak \le \varepsilon)$. In this case, however, the model parameters of both $m_{n''}$ and $m_N$ are unknown. Thus, Sample Size Estimator treats both of the model parameters as random variables and uses the joint probability distribution of $(\hat{\theta}_{n''}, \hat{\theta}_N)$, where $\hat{\theta}_{n''}$ is the random variable for the unknown model parameter $\theta_{n''}$ of $m_{n''}$. How to i.i.d.-sample from the joint probability distribution is presented in \cref{sec:sample:search}. Given the sampling mechanism that obtains the i.i.d.-samples $(\theta_{n'',i}, \theta_{N,i})$ for $i = 1, \ldots, k$, the probability $\pr(v(m_{n''}, m_N) \le \varepsilon)$ is computed using Monte Carlo simulations. This process is presented in more detail in \cref{sec:sample:quality}.

% <<<<<<< HEAD
% % \subsection{Sampling Operator}
% % \label{sec:sampling:operator}

% % \tofix{When the training set $D$ cannot fit in memory, \system can load only the necessary dataset $D_n$ from a disk or a database. For instance, when the dataset is stored as a relational table, a uniform random sample can easily be obtained using a SQL query as follows: \texttt{select * from data\_table where rand() < ratio}.
% % Although our theoretical contributions in \cref{sec:accuracy,sec:sample} are primarily developed for $D_n$ obtained by uniform random sampling, those theories rely on the asymptotic property offered by the central limit theorem; thus, those described approaches could potentially be extended to biased sampling by applying the asymptotic theory on biased sampling (also called importance sampling)~\cite{mcbook}.}
% =======
\subsection{Sampling Process}
\label{sec:sampling}

When the training set $D$ fits in memory, \system
produces $D_n$ by
simply invoking
	\tofix{\texttt{\textbf{numpy.random.choice}}} to perform uniform sampling \emph{without} replacement.
When $D$ does not fit in memory,
	\system tries to use offline samples whenever possible,
		in the form of a pre-shuffled dataset on disk (similar to~\cite{online-agg}) or a sequence of telescopic samples (similar to~\cite{mozafari_eurosys2013}).
Otherwise, \system performs
  Bernoulli sampling (as a more efficient approximation
	of uniform sampling without replacement)
 on-the-fly
 	by reading from disk or querying a SQL database.
For the latter,
 it uses the \texttt{\textbf{TABLESAMPLE}} operator when supported by the database, and
 otherwise  issues
 	the following SQL query: \texttt{\textbf{select * from D where rand() < ratio}}.
Note that, although our theoretical contributions in \cref{sec:accuracy,sec:sample} are primarily designed for uniform random sampling, our results can
	 be extended to biased (i.e., stratified) sampling by applying the asymptotic theory on biased sampling (instead of central limit theorem)~\cite{mcbook}.
}


% >>>>>>> ab19a279798c2b1f0a6a1e580a56076f63261efb


==> architecture.tex <==
\input{figures/fig_archi}

% \input{figures/fig_workflow_b}

\subsection{Architecture}
\label{sec:model:abstract}

For generality and to be agnostic to the different ML models, \system relies on an abstraction, called \emph{model class specification (\mcs)}.
We first present the common mathematical form of the ML models supported by \system, and then introduce our \mcs abstraction.
\ignore{(In \cref{sec:components}, we show how different components of \system utilize \mcs.)}

\ph{Mathematical Form}
\system currently supports any ML model that relies on maximum likelihood estimation.
Such models are trained by finding a model parameter value $\theta$ that maximizes the likelihood of the training set $D$. This optimization is equivalent to solving the following minimization problem:\footnote{We use  minimization (instead of maximization) due to the minus sign in \cref{eq:support:obj2}.}
% minimizing the following function $f_n(\theta)$:
% \tofix{including log-likelihood expressions and an optional regularization term $R(\theta)$}:

% \tofix{Jingyi: Should be argmax in eq.(1)?}

\input{figures/tab_notation}

\begin{align}
&\argmin_\theta f_n(\theta)
\label{eq:support:obj1} \\
% \end{align}
% where
% \begin{align}
\text{where} \quad
&f_n(\theta) = \frac{1}{n} \sum_{i=1}^{n}\, \minus \log \pr(\xx_i, y_i;\, \theta) + R(\theta)
\label{eq:support:obj2}
\end{align}
Here, $\pr(\xx_i, y_i;\, \theta)$ indicates the likelihood of observing the pair ($\xx_i$, $y_i$) given $\theta$, $R(\theta)$ is the optional regularization term typically used to prevent overfitting, and
$n$ is the number of training examples used. When $n$=$N$, this results in training the full model $m_N$, and otherwise we have an approximate model $m_n$.
Different ML models use different expressions for $\pr(\xx_i, y_i;\, \theta)$.
For example, PPCA uses the Gaussian distribution with covariance matrix $\xx_i \xx_i^\top$  whereas logistic regression uses
the Bernoulli distribution with its mean being the sigmoid function of $\xx_i^\top \theta$.
%\tofix{We provide their concrete examples in \cref{sec:model:abstract:example}.}


The solution $\theta_n$ to the minimization problem in \cref{eq:support:obj1}   is a value of $\theta$ at which the gradient $g_n(\theta) = \nabla f_n(\theta)$ of the objective function $f_n(\theta)$ becomes zero. That is,
% The ML models supported by \system are commonly trained by finding model parameters $\theta_n$ at which the expressions $g_n(\theta)$ as follows becomes a zero vector:
\begin{equation}
g_n(\theta_n) = \left[ \frac{1}{n} \sum_{i=1}^n q(\theta_n; \xx_i, y_i) \right] + r(\theta_n) = \bm{0}
\label{eq:abstract:model}
\end{equation}
where
	$q(\theta; \xx_i, y_i)$ denotes $\minus \nabla_\theta \log \pr(\xx_i, y_i; \theta)$ and $r(\theta)$ denotes $\nabla_\theta R(\theta)$.
% We provide concrete examples of obtaining $g_n(\theta)$ in \cref{sec:model:abstract:example}.


% \input{figures/fig_model_specification}

\ph{Model Class Specification (\mcs)} A model class specification is the abstraction that
allows \system's components to remain generic and not tied to the specific internal logic of the supported ML models.
Note that
  \system already includes the necessary \mcs definitions for the currently supported model classes (see \cref{sec:support}).
Regular users therefore do not need to provide their own \mcs.
However, more advanced developers can easily integrate new ML models (as long as they are
  	based on maximum likelihood estimation) by defining new \mcs.
To define a new \mcs in \system, the developers must inherit from the main \texttt{\textbf{ModelClass}} class and
  implement three virtual functions: \texttt{\textbf{diff()}}, \texttt{\textbf{grads()}}, and optionally, \texttt{\textbf{solve()}}.
\begin{enumerate}
\item \texttt{\textbf{diff($m_1$, $m_2$)}}: This function computes the model difference $v(m_1, m_2)$ between two models $m_1$ and $m_2$, \tofix{using part of the training set that was not used during
 model training.}
 % training either of $m_1$ and $m_2$}.
\tofix{Examples of $v(m_1, m_2)$ can be found in \cref{sec:interface}.}

% For example, for classification (e.g., logistic regression, max entropy classifier), $v(m_1, m_2) = \E[m_1(\xx) \ne m_2(\xx)]$ for $\xx \sim \mathcal{D}$. For regression (e.g., linear regression), $v(m_1, m_2) = \E[(m_1(\xx) - m_2(\xx))^2]$ for $\xx \sim \mathcal{D}$. For PPCA, $v(m_1, m_2)$ computes one minus the average cosine similarity between two models' respective extracted factors.
%
\item \texttt{\textbf{grads}}: This function returns a list of $q(\theta; \xx_i, y_i) + r(\theta)$ for $i = 1, \ldots, n$, as defined in \cref{eq:abstract:model}.
Although iterative optimization algorithms typically rely \emph{only} on the \emph{average} of this list of values (i.e., the gradient $\nabla_\theta\, f_n(\theta)$), the \texttt{grads} function must return individual values (without averaging them), as they are internally used by \system (see \cref{sec:hessian}).
%
\item \texttt{\textbf{solve}}: This optional function computes the optimal model parameters for  models that have a closed-form expression.
(Currently, \system implements the optional \texttt{solve} functions for linear regression and PPCA.)
% , as they both have closed-form solutions.)
\end{enumerate}
\cref{code:model:specification} shows an example of a model class specification.


==> exp_scale_contract.tex <==
\input{figures/fig_exp_confidence}

\subsection{Accuracy Assessment}
\label{sec:exp:assessment}

Model Accuracy Assessor (MAA) is the component used at the initial step of \system's \modea operations and is also the primary component for \system's \modeb operations. This section studies the correctness of MAA's outputs---the estimated accuracy of an approximate model.

To study MAA's correctness, we compared MAA's guaranteed accuracy of an approximate model and the actual accuracy of the approximate model. Our comparisons were made for three different combinations of a model and a dataset, i.e., (LR, \higgs), (ME, \mnist), and (PPCA, \mnist); and for different sample sizes of training sets (on which approximate models were trained).

\cref{fig:exp:accuracy} shows our experiment results. Observe that the gaps between the actual accuracies and the guaranteed accuracies were larger when the sample sizes were relatively small. This is because when sample sizes were small, the variances of approximate models (or accurately, the variances of the outputs of approximate models) were estimated high; thus, MAA was more conservative to ensure the correctness of its outputs. The gap decreased as the sample sizes increased. In all cases, however, the actual accuracies of approximate models were higher than MAA's guaranteed accuracies, which indicates the correctness of MAA.


==> exp_statistics.tex <==
%!TEX root = approx_ml.tex

% \input{figures/tab_exp_hessian}

\subsection{Statistics Computation}
\label{sec:exp:hessian}

% In \cref{sec:hessian}, we presented two general
% methods---InverseGradients and ObservedFisher---for computing important statistics, i.e., $H$ and $J$.

In this section, we compare ClosedForm, InverseGradients, ObservedFisher in terms of both accuracy and efficiency.
 This analysis serves as an empirical justification of why ObservedFisher is \system's default choice.

\ph{Accuracy}
\tofix{In this section, we compare the accuracy of the three methods using (Lin, \power) for different sample sizes. To compute the accuracy, we measured the ratio of the average estimated variance of parameters (by each method) to the average true variance of parameters. It is desirable that the estimates are conservative (ratio being not smaller than 1.0) while being close to the true values (ratio being close to 1.0).
\cref{sec:exp:statistics} shows the result. In general, ClosedForm was the most accurate while ObservedFisher was the least accurate.
However, as the number of sample size increases, the accuracies of those methods increased in general (i.e., ratio becoming close to 1.0); also, the accuracy of ObservedFisher was comparable to other methods. Recall that ClosedForm is available for only certain models (e.g., Lin and LR) while InverseGradients and ObservedFisher are available for all supported models. Below, we compare InverseGradients and ObservedFisher in more detail with other models.
}


\ph{Efficiency}
To compare InverseGradients and ObservedFisher in depth, we used two more combinations (LR, \higgs) and (ME, \mnist). Recall from \cref{tab:datasets} that \higgs is a low-dimensional dataset ($d = 28$) while \mnist is high-dimensional ($d = 784$).
This difference in number of dimensions reveals interesting properties regarding InverseGradients versus ObservedFisher.
We used each method to compute the covariance matrix $H^{\minus 1} J H^{\minus 1}$ (which determines the parameter distribution in \cref{thm:param_dist}, \cref{sec:accuracy}).
We measured the runtime of each method and calculated the accuracy of its estimated covariance matrix.
To measure the accuracy, we calculated the average Frobenius norm, i.e., $(1/d^2)\, \|C_t - C_e\|_F$,
 where $C_t$ was the true covariance matrix and $C_e$ was the estimated covariance matrix.

\tofix{\cref{tab:datasets} summarizes} the results of this experiment. For the low-dimensional data (\higgs), the runtimes and the accuracies of the two methods were comparable. However, their performance differed much for the high-dimensional data (\mnist). Since InverseGradients had to invoke the \texttt{grads} function repeatedly (i.e., $d$ times), its runtime  increased significantly.
In contrast, ObservedFisher had to call the \texttt{grads} function only once.
However, their accuracies remained comparable even for the high-dimensional data.



==> figures/algo_training.tex <==
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\begin{algorithm}
\caption{Learning Error-bounded Model Parameters}
\label{algo:training}

\begin{algorithmic}[1]
\Procedure{MyProcedure}{}
\State $\textit{stringlen} \gets \text{length of }\textit{string}$
\State $i \gets \textit{patlen}$
\BState \emph{top}:
\If {$i > \textit{stringlen}$} \Return false
\EndIf
\State $j \gets \textit{patlen}$
\BState \emph{loop}:
\If {$\textit{string}(i) = \textit{path}(j)$}
\State $j \gets j-1$.
\State $i \gets i-1$.
\State \textbf{goto} \emph{loop}.
\State \textbf{close};
\EndIf
\State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
\State \textbf{goto} \emph{top}.
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> figures/bootstrap_error_bound_size.tex <==
\begin{figure}[t]
  \pgfplotsset{subsampling/.style={
    % width=47mm,
    % height=35mm,
    % ymax=1.4,
    % ymin=0,
    x post scale=0.5,
    y post scale=0.5,
    % xmin=1,
    % xmax=6,
    % ylabel=Standard Deviation,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    % xtick={1,2,3,4,5,6,7,8},
    % xticklabels={t1,t9,t12,t15,t17,c1,c2,c3},
    % ytick={0, 50, 100},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    % ylabel shift=-3pt,
    % xlabel shift=-2pt,
    legend style={
        at={(0,1.14)},
        anchor=south west,%column sep=2pt,
        scale=0.8,
        draw=black,fill=none,line width=.5pt,
        % /tikz/every even column/.append style={column sep=40pt}
    },
    % legend style={
    %   at={(0, 1)},
    %   anchor=north west,
    %   fill=none,
    %   scale=0.8,
    % },
    % legend columns=2,
    % every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\tiny}
  }}

  \centering
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 6},
        xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,},
        xlabel=Sampling Ratio,
        ylabel=Model Error Bound Size,
        % ymode=log,
        colormap/cool,
      ]
      \addplot[color=myblue,mark=*,mark size=1.5]
      coordinates {
        (1,0.0108) (2,0.0079) (3,0.0051) (4,0.0036) (5,0.0026) (6,0.0016)
      };
      \addlegendentry{Logistic Model Error}
      \addplot[color=myred,mark=+,mark size=1.5]
      coordinates{
        (1,0.0455) (2,0.0385) (3,0.0195) (4,0.0193) (5,0.0117) (6,0.0069)
      };
      \addlegendentry{Linear Model Error}
      \end{axis}
    \end{tikzpicture}
  \end{subfigure}
  ~
  \centering
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 6},
        xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,},
        xlabel=Sampling Ratio,
        ylabel=Prediction Error Bound Size,
        % ymode=log,
        colormap/cool,
      ]
        \addplot[color=myblue,mark=*,mark size=1.5]
        coordinates{
          (1,0.000000515151515) (2,0.000001090909091) (3,0.000000060606061) (4,0) (5,0) (6,0)
        };
        \addlegendentry{Logistic Prediction Error}
        \addplot[color=myred,mark=+,mark size=1.5]
        coordinates{
          (1, 1.2291) (2, 0.8810) (3, 0.5394) (4, 0.3869) (5, 0.2818) (6, 0.1764)
        };
        \addlegendentry{Linear Prediction Error}
      \end{axis}
    \end{tikzpicture}
  \end{subfigure}
  \caption{Average Size of Error Bound in Bootstrap for Different Sampling Ratios}
  \label{fig:error_bound_size}
\end{figure}

==> figures/bootstrap_model_error_bound_prob.tex <==
\begin{figure}[t]
  \pgfplotsset{subsampling/.style={
    % width=47mm,
    % height=35mm,
    % ymax=1.4,
    % ymin=0.6,
    x post scale=0.5,
    y post scale=0.5,
    % xmin=1,
    % xmax=6,
    % ylabel=Standard Deviation,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    % xtick={1,2,3,4,5,6,7,8},
    % xticklabels={t1,t9,t12,t15,t17,c1,c2,c3},
    % ytick={0, 50, 100},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    % ylabel shift=-3pt,
    % xlabel shift=-2pt,
    legend style={
        at={(0,1.04)},
        anchor=south west,%column sep=2pt,
        scale=0.8,
        draw=black,fill=none,line width=.5pt,
        % /tikz/every even column/.append style={column sep=40pt}
    },
    % legend style={
    %   at={(0, 1)},
    %   anchor=north west,
    %   fill=none,
    %   scale=0.8,
    % },
    legend columns=2,
    % every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\tiny}
  }}

  \centering
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 7},
        xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,100\%,},
        xlabel=Sampling Ratio,
        % ylabel=Probability of Error Bound Holding for Sample Model (\%),
      ]
        \addplot[color=darkorange,mark=triangle,mark size=1.5]
        coordinates{
          (1, 100) (2, 100) (3, 100) (4, 100) (5, 100) (6, 100)
        };
      \end{axis}
    \end{tikzpicture}
    \caption{Bootstrap Logistic Regression}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 7},
        xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,100\%,},
        xlabel=Sampling Ratio,
        % ylabel=Probability of Error Bound Holding for Sample Model (\%),
      ]
        \addplot[color=darkorange,mark=triangle,mark size=1.5]
        coordinates{
          (1, 100) (2, 100) (3, 100) (4, 100) (5, 100) (6, 100)
        };
      \end{axis}
    \end{tikzpicture}
    \caption{Bootstrap Linear Regression}
  \end{subfigure}

  \caption{Probability of Model Error Bound Holding (\%)}
  \label{fig:model_error_bound_prob}
\end{figure}

==> figures/bootstrap_prediction_error_bound_prob.tex <==
\begin{figure}[t]
  \pgfplotsset{subsampling/.style={
    % width=47mm,
    % height=35mm,
    % ymax=1.4,
    % ymin=0.6,
    x post scale=0.5,
    y post scale=0.5,
    % xmin=1,
    % xmax=6,
    % ylabel=Standard Deviation,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    % xtick={1,2,3,4,5,6,7,8},
    % xticklabels={t1,t9,t12,t15,t17,c1,c2,c3},
    % ytick={0, 50,0},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    % ylabel shift=-3pt,
    % xlabel shift=-2pt,
    legend style={
        at={(0,1.04)},
        anchor=south west,%column sep=2pt,
        scale=0.8,
        draw=black,fill=none,line width=.5pt,
        % /tikz/every even column/.append style={column sep=40pt}
    },
    % legend style={
    %   at={(0, 1)},
    %   anchor=north west,
    %   fill=none,
    %   scale=0.8,
    % },
    legend columns=2,
    % every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\tiny}
  }}

  \centering
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 7},
        xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,100\%,},
        xlabel=Sampling Ratio,
      ]
        \addplot[color=darkorange,mark=triangle,mark size=1.5]
        coordinates{
          (1,0) (2,0) (3,0) (4,0) (5,0) (6,0)
        };
      \end{axis}
    \end{tikzpicture}
    \caption{Logistic Regression}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 7},
        xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,100\%,},
        xlabel=Sampling Ratio,
      ]
        \addplot[color=darkorange,mark=triangle,mark size=1.5]
        coordinates{
          (1,0) (2,0) (3,0) (4,0) (5,0) (6,0)
        };
      \end{axis}
    \end{tikzpicture}
    \caption{Linear Regression}
  \end{subfigure}

  \caption{Probability of Prediction Error Bound Holding (\%)}
  \label{fig:prediction_error_bound_prob}
\end{figure}

==> figures/delta_bounding_prob.tex <==
\begin{figure}[t]
  \pgfplotsset{subsampling/.style={
    % width=47mm,
    % height=35mm,
    % ymax=1.4,
    % ymin=0,
    x post scale=0.5,
    y post scale=0.5,
    % xmin=1,
    % xmax=6,
    % ylabel=Standard Deviation,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    % xtick={1,2,3,4,5,6,7,8},
    % xticklabels={t1,t9,t12,t15,t17,c1,c2,c3},
    % ytick={0, 50, 100},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    % ylabel shift=-3pt,
    % xlabel shift=-2pt,
    legend style={
        at={(0,1.04)},
        anchor=south west,%column sep=2pt,
        scale=0.8,
        draw=black,fill=none,line width=.5pt,
        % /tikz/every even column/.append style={column sep=40pt}
    },
    % legend style={
    %   at={(0, 1)},
    %   anchor=north west,
    %   fill=none,
    %   scale=0.8,
    % },
    legend columns=2,
    % every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\tiny}
  }}

  \centering
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 5},
        xticklabels={0.01,0.02,0.05,0.1,0.2,},
        xlabel=Value of $\delta$,
        % ylabel=Model Error Bound Size,
        % ymode=log,
        colormap/cool,
      ]
      \addplot[color=darkorange,mark=*,mark size=1.5]
      coordinates {
        (1,100) (2,100) (3,100) (4,100) (5,100)
      };
      \end{axis}
    \end{tikzpicture}
  \caption{Logistic Regression}
  \end{subfigure}
  ~
  \centering
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[subsampling,
        xtick={1, 2, ..., 5},
        xticklabels={0.01,0.02,0.05,0.1,0.2,},
        xlabel=Value of $\delta$,
        % ylabel=Prediction Error Bound Size,
        % ymode=log,
        colormap/cool,
      ]
      \addplot[color=darkorange,mark=*,mark size=1.5]
      coordinates {
        (1,100) (2,100) (3,100) (4,100) (5,100)
      };
      \end{axis}
    \end{tikzpicture}
  \caption{Linear Regression}
  \end{subfigure}
  \caption{Probability of Erorr Bound Holding for Sample Prediction Under Different Values of $\delta$ (\%)}
  \label{fig:delta_error_bound_prob}
\end{figure}

==> figures/fig_code.tex <==
\begin{figure}[t]

\begin{subfigure}[b]{\linewidth}
\begin{lstlisting}[
	language=Python,
    basicstyle=\color{vintageblack}\small\ttfamily,
    xleftmargin=15pt,
    commentstyle=\color{vintagegreen},
    morekeywords={fit},
    keywordstyle=\bfseries,
    classoffset=1,
    morekeywords={sklearn, sml},
    keywordstyle=\bfseries\color{vintageorange},
    classoffset=0,
    numbers=left,
    stepnumber=1,
    % caption={Using \system.},captionpos=b,
    % label={fig:code:train}
]
from sklearn import linear_model as sml
lr = sml.LogisticRegression()
model = lr.fit(features, labels)
\end{lstlisting}

\vspace{-3mm}
\caption{scikit-learn}
\label{fig:code:sklearn}
\end{subfigure}

\vspace{2mm}

\begin{subfigure}[b]{\linewidth}
\begin{lstlisting}[
    language=Python,
    basicstyle=\color{vintageblack}\small\ttfamily,
    xleftmargin=15pt,
    commentstyle=\color{vintagegreen},
    morekeywords={fit},
    keywordstyle=\bfseries,
    classoffset=1,
    morekeywords={anonsys, asys, ApproxContract},
    keywordstyle=\bfseries\color{vintageorange},
    classoffset=0,
    numbers=left,
    stepnumber=1,
    % caption={Using \system.},captionpos=b,
    % label={fig:code:train}
]
import anonsys as asys
lr = asys.LogisticRegression()
ap = asys.ApproxContract(e=0.01, d=0.05)
model = lr.fit(features, labels, ap)
\end{lstlisting}

\vspace{-3mm}
\caption{\system (\modea)}
\label{fig:code:ours:a}
\end{subfigure}

\vspace{2mm}

\begin{subfigure}[b]{\linewidth}
\begin{lstlisting}[
    language=Python,
    basicstyle=\color{vintageblack}\small\ttfamily,
    xleftmargin=15pt,
    commentstyle=\color{vintagegreen},
    morekeywords={fit},
    keywordstyle=\bfseries,
    classoffset=1,
    morekeywords={anonsys, asys, ApproxContract},
    keywordstyle=\bfseries\color{vintageorange},
    classoffset=0,
    numbers=left,
    stepnumber=1,
    % caption={Using \system.},captionpos=b,
    % label={fig:code:train}
]
import anonsys as asys
lr = asys.LogisticRegression()
ap = asys.ApproxContract(n=10000, d=0.05)
model = lr.fit(features, labels, ap)
\end{lstlisting}

\vspace{-3mm}
\caption{\system (\modeb)}
\label{fig:code:ours:b}
\end{subfigure}

\vspace{-2mm}
\caption{Examples of training a model in a typical ML library (scikit-learn in this case) versus \system.}
\label{fig:code}
\end{figure}

==> figures/fig_exp_comp_baseline.tex <==
\begin{figure*}[t]

\pgfplotsset{compbase/.style={
        width=60mm,
        height=40mm,
        xmin=0.5,
        xmax=5.5,
        ymin=0,
        ymax=240,
        xlabel=Requested Model Agreement ($(1-\delta) \times 100$\%),
        ylabel=Training Time,
        xlabel near ticks,
        ylabel near ticks,
        ylabel style={align=center},
        xtick={1, 2, 3, 4, 5},
        xticklabels={90\%, 95\%, 99\%, 99.5\%, 99.9\%},
        % ytick={0, 1800, 3600, 5400, 7200},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        ytick={0, 60, 120, 180, 240},
        yticklabels={0 min, 1 min, 2 min, 3 min, 4 min},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        % extra y ticks={10, 20, 30, 40},
        % extra y tick style={yticklabels={}},
        ylabel shift=-3pt,
        % xlabel shift=-2pt,
        legend style={
            at={(0,1.05)},anchor=south west,column sep=2pt,
            draw=black,fill=none,line width=.5pt,
            /tikz/every even column/.append style={column sep=20pt}
        },
        legend columns=2,
        every axis/.append style={font=\footnotesize},
        ymajorgrids,
        % yminorgrids,
        minor grid style=lightgray,
        % nodes near coords,
        % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
    }}

\centering
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[compbase]

\addplot[mark=*,mark size=1.5,mark options={fill=vintageorange},
ultra thick,draw=vintageorange,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  0.01  0.01\%
2  0.12  0.12\%
3  2.00  2.00\%
4  6.93  6.93\%
5  6.40  6.40\%
% 6  6060 {1.68 hr}
};

\addplot[mark=*,mark size=1.5,mark options={fill=vintagegreen},
ultra thick,draw=vintagegreen,point meta = explicit symbolic]
table[x=x,y=y] {
x y
1  1.12  
2  2.79  
3 31.92  
4 39.29  
5 41.20  
% 6  6060 {1.68 hr}
};

\addlegendentry{\higgs}
\addlegendentry{\yelp}

% \draw[vintageorange,thick] (axis cs:0.5,6060) -- (axis cs:5.5,6060);

\end{axis}
\end{tikzpicture}
\caption{Logistic Regression}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[compbase]
\end{axis}
\end{tikzpicture}
\caption{Max Entropy Classifier}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[compbase]
\end{axis}
\end{tikzpicture}
\caption{PPCA}
\end{subfigure}

\caption{\system's training time compared to baseline sampling-based training methods.}
\end{figure*}


==> figures/fig_exp_confidence.tex <==
\begin{figure*}[t]

\vspace{2mm}
\pgfplotsset{confest/.style={
    width=58mm,
    height=35mm,
    % ybar,
    % bar width=1.5mm,
    xmin=0.5,
    xmax=8.5,
    ymin=75,
    ymax=100,
    xlabel=Sample Size ($n$),
    ylabel=Accuracy (\%),
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    xtick={1, 2, ..., 8},
    xticklabels={2K, 4K, 8K, 10K, 12K, 14K, 18K, 20K},
    % ytick={0, 1800, 3600, 5400, 7200},
    % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
    ytick={75, 80, ..., 100},
    yticklabels={75\%, 80\%, 85\%, 90\%, 95\%, 100\%},
    % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    ylabel shift=-3pt,
    % xlabel shift=-2pt,
    legend style={
        at={(0,1.1)},anchor=south west,column sep=2pt,
        draw=black,fill=white,line width=.5pt,
        /tikz/every even column/.append style={column sep=20pt}
    },
    legend columns=2,
    every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}

\centering
\begin{subfigure}[t]{0.32\textwidth}
\begin{tikzpicture}
\begin{axis}[confest]

\addplot[mark=*,mark size=1.5,ultra thick,draw=vintageorange,
mark options={fill=vintageorange}]
table[x=x,y=y] {
x y
1  82.24
2  88.00
3  91.05
4  91.75
5  92.50
6  93.60
7  93.60
8  94.05
};

\addplot[mark=*,mark size=1.5,ultra thick,draw=vintagegreen,
mark options={fill=vintagegreen}]
table[x=x,y=y] {
x y
1  86.790
2  90.360
3  94.255
4  93.510
5  95.085
6  95.905
7  95.045
8  94.390
};

\addlegendentry{\system's Guaranteed Model Accuracy}
\addlegendentry{Actual Model Accuracy}

% \draw[vintageorange,thick] (axis cs:0.5,6060) -- (axis cs:5.5,6060);

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{LR, \higgs}
\end{subfigure}
~
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[confest,
ytick={65, 70, ..., 90},
yticklabels={65\%, 70\%, 75\%, 80\%, 85\%, 90\%},
ymin=65,
ymax=90,
]

\addplot[mark=*,mark size=1.5,ultra thick,draw=vintageorange,
mark options={fill=vintageorange}]
table[x=x,y=y] {
x y
1  70.15
2  75.90
3  77.85
4  80.85
5  82.40
6  83.05
7  84.75
8  85.75
};

\addplot[mark=*,mark size=1.5,ultra thick,draw=vintagegreen,
mark options={fill=vintagegreen}]
table[x=x,y=y] {
x y
1  70.80
2  72.40
3  80.10
4  80.20
5  81.10
6  84.90
7  86.70
8  86.90
};

% \addlegendentry{\system's Estimates}
% \addlegendentry{Actual Accuracy}
\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{ME, \yelp}
\end{subfigure}
~
\begin{subfigure}[t]{0.32\textwidth}
\begin{tikzpicture}
\begin{axis}[confest]

\addplot[mark=*,mark size=1.5,ultra thick,draw=vintageorange,
mark options={fill=vintageorange}]
table[x=x,y=y] {
x y
1  79.98
2  89.17
3  94.09
4  94.85
5  96.05
6  96.76
7  97.22
8  97.81
};

\addplot[mark=*,mark size=1.5,ultra thick,draw=vintagegreen,
mark options={fill=vintagegreen}]
table[x=x,y=y] {
x y
1  94.90
2  96.52
3  98.91
4  99.20
5  99.26
6  99.27
7  99.21
8  99.49
};

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{PPCA, \mnist}
\end{subfigure}

\vspace{-2mm}
\caption{The correctness of \system's model accuracy assessment. The assessed (i.e., guaranteed) model accuracies are compared to the actual model accuracies.
In all cases, the actual model accuracies were higher than the guaranteed accuracies.
}
\label{fig:exp:accuracy}
\vspace{2mm}
\end{figure*}


==> figures/fig_exp_runtime_analysis.tex <==
\pgfplotsset{runtimeanalysis/.style={
        width=75mm,
        height=30mm,
        xmin=0,
        xmax=500,
        ymin=0.5,
        ymax=2.5,
        xbar stacked,
        bar width=2mm,
        xlabel=Runtime,
        % ylabel=Relative\\ Training Time (\%),
        xlabel near ticks,
        ylabel near ticks,
        ylabel style={align=center},
        xtick={0, 100, ..., 500},
        xticklabels={0 sec, 100 sec, 200 sec, 300 sec, 400 sec, 500 sec},
        ytick={1, 2},
        yticklabels={ME on \mnist, LR on \yelp},
        ylabel shift=-3pt,
        % xlabel shift=-2pt,
        legend style={
            at={(0,1.05)},anchor=south west,column sep=2pt,
            draw=black,fill=white,line width=.5pt,
            /tikz/every even column/.append style={column sep=5pt}
        },
        legend cell align={left},
        legend columns=2,
        every axis/.append style={font=\footnotesize},
        xmajorgrids,
        % yminorgrids,
        minor grid style=lightgray,
        % nodes near coords,
        % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
    }}

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.48\textwidth}
% \centering
\begin{tikzpicture}
\begin{axis}[runtimeanalysis]
% y=2 LR+HIGGS
% y=1 ME+MNIST

% initial training
\addplot[draw=vintageblack!50!white,fill=vintageblack!50!white]
table[x=x,y=y] {
x y
1.74 2
52.97 1
};

% Inverse Hessian
\addplot[draw=vintageorange,fill=vintageorange]
table[x=x,y=y] {
x y
0.22 2
1.09 1
};

% Search
\addplot[draw=vintagegreen,fill=vintagegreen]
table[x=x,y=y] {
x y
1.35 2
17.91 1
};

% Final Model
\addplot[draw=vintageblack,fill=vintageblack]
table[x=x,y=y] {
x y
26.93 2
408.23 1
};

\addlegendentry{Initial Training}
\addlegendentry{Statistics Computation}
\addlegendentry{Sample Size Searching}
\addlegendentry{Final Training}

\end{axis}
\end{tikzpicture}
\caption{\modea: The requested confidence was 95\%.}
\label{fig:exp:runtime:a}
\end{subfigure}
%
%
\quad
%
%
\begin{subfigure}[b]{0.48\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[runtimeanalysis,
xmax=60,
xtick={0, 15, ..., 60},
xticklabels={0 sec, 15 sec, 30 sec, 45 sec, 60 sec},
]
% y=2 LR+HIGGS
% y=1 ME+MNIST

% initial training
\addplot[draw=vintageblack,fill=vintageblack]
table[x=x,y=y] {
x y
1.74 2
52.97 1
};

% Inverse Hessian
\addplot[draw=vintageorange,fill=vintageorange]
table[x=x,y=y] {
x y
0.22 2
1.09 1
};

% Search
\addplot[draw=vintagegreen,fill=vintagegreen]
table[x=x,y=y] {
x y
0.28 2
0.55 1
};


\addlegendentry{Model Training}
\addlegendentry{Statistics Computation}
\addlegendentry{Accuracy Estimation}

\end{axis}
\end{tikzpicture}
\caption{\modeb: The specified sample size was 10,000.}
\label{fig:exp:runtime:b}
\end{subfigure}

\vspace{-2mm}
\caption{\system's training time decomposition for both \modea and \modeb. \system's runtime overhead for computing necessary statistics, searching minimum sample sizes, and estimating confidence were small compared to the overall training time. }
\label{fig:exp:runtime}
\end{figure*}


==> figures/fig_exp_sss.tex <==
\begin{figure*}[t]

\pgfplotsset{sss/.style={
        width=58mm,
        height=35mm,
        xmin=1.5,
        xmax=6.5,
        ymin=0,
        ymax=100,
        xlabel=Requested Accuracy ($(1-\varepsilon) \times 100$\%),
        ylabel=Sample Size,
        xlabel near ticks,
        ylabel near ticks,
        ylabel style={align=center},
        xtick={1, 2, 3, 4, 5, 6},
        xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
        % ytick={0, 1800, 3600, 5400, 7200},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        ytick={0, 20, ..., 100},
        yticklabels={0\%, 20\%, 40\%, 60\&, 80\%, 100\%},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        % extra y ticks={10, 20, 30, 40},
        % extra y tick style={yticklabels={}},
        ylabel shift=-3pt,
        xlabel shift=-2pt,
        legend style={
            at={(0,1.1)},anchor=south west,column sep=2pt,
            draw=black,fill=none,line width=.5pt,
            /tikz/every even column/.append style={column sep=20pt}
        },
        legend cell align={left},
        legend columns=3,
        every axis/.append style={font=\footnotesize},
        ymajorgrids,
        xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
        % yminorgrids,
        % minor grid style=lightgray,
        % nodes near coords,
        % every node near coord/.append style={font=\footnotesize,rotate=0}
        scaled y ticks=false
    }}

\centering
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[sss,
]

\addplot[mark=triangle*,mark size=2.5,ultra thick,draw=vintagegreen,
mark options={fill=vintagegreen}]
table[x=x,y=y] {
x y
% 1     1000
2  0.01
3  0.01
4  0.02
5  0.42
6  1.68
};

\addplot[mark=*,mark size=2,ultra thick,draw=vintageorange,
mark options={fill=vintageorange}]
table[x=x,y=y] {
x y
% 1    10000
2  0.01
3  0.01
4  0.04
5  1.17
6  4.69
};


\addlegendentry{\gradual}
\addlegendentry{\system}

% \addlegendimage{mark=*,mark size=1.5,ultra thick,dashed,draw=vintagegreen,
% mark options={fill=vintagegreen}}
% \addlegendentry{\gradual (projected due to timeout)}

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{LR, \higgs}
\end{subfigure}
~
\begin{subfigure}[t]{0.32\textwidth}
\centering
% \vspace{3mm}
\begin{tikzpicture}
\begin{axis}[sss,
% ymin=0,
% ymax=10000000,
% ytick={0,2000000,4000000,6000000,8000000,10000000},
% yticklabels={0, 2M, 4M, 6M, 8M, 10M},
]

\addplot[mark=triangle*,mark size=2.5,ultra thick,draw=vintagegreen,
mark options={fill=vintagegreen}]
table[x=x,y=y] {
x y
% 1    9000
2  0.16
3  0.49
4  2.25
5  64.0
};


\addplot[mark=*,mark size=2,ultra thick,draw=vintageorange,
mark options={fill=vintageorange}]
table[x=x,y=y] {
x y
% 1    23453
2  0.63
3  1.51
4  5.64
5  60.6
6  86.2
};

% \addplot[mark=*,mark size=1.5,ultra thick,draw=vintagegreen,
% mark options={fill=vintagegreen}]
% table[x=x,y=y] {
% x y
% % 1    9000
% 2   16000
% 3   49000
% 4  225000
% 5  6400000
% % 6  0
% };


% \addplot[mark=*,mark size=1.5,ultra thick,draw=vintageorange,
% mark options={fill=vintageorange}]
% table[x=x,y=y] {
% x y
% % 1    23453
% 2    62591
% 3   150622
% 4   563784
% 5  6060729
% 6  8615240
% };

% \addplot[mark=*,mark size=1.5,ultra thick,dashed,draw=vintagegreen,
% mark options={fill=vintagegreen}]
% table[x=x,y=y] {
% x y
% 4  0
% 5  6400000
% 6  7500000
% };

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{ME, \yelp}
\end{subfigure}
~
\begin{subfigure}[t]{0.32\textwidth}
\centering
% \vspace{3mm}
\begin{tikzpicture}
\begin{axis}[sss,
xmax=7.5,
xtick={1, 2, 3, 4, 5, 6, 7},
% xticklabels={0.90, 0.95, 0.99, 0.995, 0.999, 0.9995, 0.9999},
xticklabels={90\%, 95\%, 99\%, 99.5\%, 99.9\%, 99.95\%, 99.99\%},
% xlabel shift=0mm,
xlabel=Requested Accuracy ($(1-\varepsilon) \times 100\%$),
% ymin=0,
% ymax=2500000,
% ytick={0,500000,1000000,1500000,2000000,2500000},
% yticklabels={0, 0.5M, 1.0M, 1.5M, 2.0M, 2.5M},
]

\addplot[mark=triangle*,mark size=2.5,ultra thick,draw=vintagegreen,
mark options={fill=vintagegreen}]
table[x=x,y=y] {
x y
% 1     4000
2  0.09
3  0.49
4  1.21
5  4.41
6  6.76
7  22.1
};

\addplot[mark=*,mark size=2,ultra thick,draw=vintageorange,
mark options={fill=vintageorange}]
table[x=x,y=y] {
x y
% 1     2785
2  0.06
3  0.27
4  0.54
5  2.56
6  4.85
7  16.6
};

% \addplot[mark=*,mark size=1.5,ultra thick,draw=vintagegreen,
% mark options={fill=vintagegreen}]
% table[x=x,y=y] {
% x y
% % 1     4000
% 2     9000
% 3    49000
% 4   121000
% 5   441000
% 6   676000
% 7  2209000
% };

% \addplot[mark=*,mark size=1.5,ultra thick,draw=vintageorange,
% mark options={fill=vintageorange}]
% table[x=x,y=y] {
% x y
% % 1     2785
% 2     5531
% 3    27224
% 4    54134
% 5   256239
% 6   484703
% 7  1663136
% };

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{PPCA, \mnist}
\label{fig:exp:sss:d}
\end{subfigure}

\vspace{-2mm}
\caption{Goodness of \system's estimated minimum sample sizes. \system's estimated minimum sample sizes were compared to the minimum sample sizes determined by \gradual.
The minimum sample sizes estimated by \system were close to the ones determined by \gradual, a slow incremental searching technique.}
\label{fig:exp:sss}
\end{figure*}


==> figures/fig_exp_time_saving2.tex <==
\begin{figure*}[t]

\pgfplotsset{timesavingg/.style={
        width=60mm,
        height=35mm,
        ybar,
        bar width=1.3mm,
        xmin=0.5,
        xmax=5.5,
        ymin=0,
        ymax=600,
        xlabel=Requested Model Agreement ($(1-\delta) \times 100$\%),
        ylabel=Training Time,
        xlabel near ticks,
        ylabel near ticks,
        ylabel style={align=center},
        xtick={1, 2, 3, 4, 5},
        xticklabels={90\%, 95\%, 99\%, 99.5\%, 99.9\%},
        % ytick={0, 1800, 3600, 5400, 7200},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        ytick={0, 120, ..., 600},
        yticklabels={0 min, 2 min, 4 min, 6 min, 8 min, 10 min},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        % extra y ticks={10, 20, 30, 40},
        % extra y tick style={yticklabels={}},
        ylabel shift=-3pt,
        % xlabel shift=-2pt,
        legend style={
            at={(0,1.1)},anchor=south west,column sep=2pt,
            draw=black,fill=none,line width=.5pt,
            /tikz/every even column/.append style={column sep=10pt}
        },
        legend cell align={left},
        legend columns=3,
        every axis/.append style={font=\footnotesize},
        ymajorgrids,
        % yminorgrids,
        minor grid style=lightgray,
        nodes near coords,
        every node near coord/.append style={font=\footnotesize,rotate=0}
    }}

\centering
\begin{subfigure}[b]{0.32\textwidth}
% \centering
\begin{tikzpicture}
\begin{axis}[timesavingg]

\addplot[fill=vintageblack,draw=vintageblack,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  0.3  {}
2  2.0  {}
3  31.0 {}
4  80   {}
5  0    {}
};

\addplot[fill=vintagegreen,draw=vintagegreen,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  1.0    {}
2  4.2    {}
3  56.3   {}
4  136.3  {}
5  0      {}
};

\addplot[fill=vintageorange,draw=vintageorange,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  0.64    0.01\%
2  7.20    0.12\%
3  121.14  2.00\%
4  420.23  6.93\%
5  387.76  6.40\%
};

\addlegendentry{OracleEst + OracleSearch}
\addlegendentry{OracleEst + ExponentialSearch}
\addlegendentry{\system}

\node[anchor=north west] at (axis cs: 0,600) {\%: ratio to full training};

% \draw[vintageorange,thick] (axis cs:0.5,6060) -- (axis cs:5.5,6060);

\end{axis}
\end{tikzpicture}
\caption{Logistic Regression}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[timesavingg]
\end{axis}
\end{tikzpicture}
\caption{Max Entropy Classifier}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[timesavingg]
\end{axis}
\end{tikzpicture}
\caption{PPCA}
\end{subfigure}

\caption{\system's training time compared to the impossibly ideal system---Oracle (note: not a database system). OracleEst indicates the ability to exactly compute the model agreement between a sample-based model and a full model. OracleSearch indicates the ability to pinpoint the minimum sample size sufficiently large to meet a requested quality guarantee.}
\end{figure*}


==> figures/fig_model_specification.tex <==
\begin{figure}[t]

\begin{lstlisting}[
	language=Python,
    basicstyle=\color{vintageblack}\small\ttfamily,
    xleftmargin=15pt,
    commentstyle=\color{vintagegreen},
    morekeywords={fit},
    keywordstyle=\bfseries,
    classoffset=1,
    morekeywords={ModelClass,diff,grads,solve,LogisticRegressionModel},
    deletekeywords={object},
    keywordstyle=\bfseries\color{vintageorange},
    classoffset=0,
    numbers=left,
    stepnumber=1,
    % caption={Using \system.},captionpos=b,
    % label={fig:code:train}
]
class LogisticRegressionModel(MCS):
  def __init__(self, config):
    self._config = config

  def diff(self, model1, model2, holdout):
    # Computes misclassification ratio.
    # @param holdout Holdout training set
    y1 = model1.predict(holdout)
    y2 = model2.predict(holdout)
    return numpy.mean(y1 != y2)

  def grads(self, theta, features, labels):
    # Computes per-example gradients
    q = sigmoid(features.dot(theta)-labels)
    q = features * q
    r = self._c.beta * theta
    return q + r
\end{lstlisting}

\vspace{-2mm}
\caption{Example of a model class specification (MCS)}
\label{code:model:specification}
\end{figure}


% def solve(self, features, labels):
%   # If available, this method directly
%   # computes optimal parameter values.
%   raise NotImplementedError

==> figures/fig_time_saving_old.tex <==
\begin{figure*}[t]

\pgfplotsset{timesaving/.style={
        width=58mm,
        height=35mm,
        xmin=0.5,
        xmax=6.5,
        ymin=0,
        ymax=100,
        xlabel=Requested Accuracy ($(1-\varepsilon) \times 100$\%),
        ylabel=Relative\\ Training Time (\%),
        xlabel near ticks,
        ylabel near ticks,
        ylabel style={align=center},
        xtick={1, 2, 3, 4, 5, 6},
        xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
        xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
        % ytick={0, 1800, 3600, 5400, 7200},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        ytick={0, 20, ..., 100},
        yticklabels={0\%, 20\%, 40\%, 60\%, 80\%, 100\%},
        % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
        % extra y ticks={10, 20, 30, 40},
        % extra y tick style={yticklabels={}},
        ylabel shift=-3pt,
        xlabel shift=-2pt,
        legend style={
            at={(0,1)},anchor=north west,column sep=2pt,
            draw=black,fill=white,line width=.5pt,
            /tikz/every even column/.append style={column sep=20pt}
        },
        legend columns=1,
        legend cell align={left},
        every axis/.append style={font=\footnotesize},
        ymajorgrids,
        % yminorgrids,
        minor grid style=lightgray,
        % nodes near coords,
        % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
    }}

\centering
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[timesaving]

\addplot[mark=*,mark size=1.5,mark options={fill=vintageorange},
ultra thick,draw=vintageorange,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  0.01  0.01\%
2  0.01  0.01\%
3  0.01  0.01\%
4  0.05  0.05\%
5  2.43  2.43\%
6  8.02  8.02\%
};

\addplot[mark=*,mark size=1.5,mark options={fill=vintagegreen},
ultra thick,draw=vintagegreen,point meta = explicit symbolic]
table[x=x,y=y] {
x y
1  00.27  00.27\%
2  00.27  00.27\%
3  03.32  03.32\%
4  07.49  07.49\%
5  34.16  34.16\%
6  66.58  66.58\%
};

\addlegendentry{\higgs}
\addlegendentry{\yelp}

% \draw[vintageorange,thick] (axis cs:0.5,6060) -- (axis cs:5.5,6060);

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{Logistic Regression (LR)}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[timesaving]
\addplot[mark=*,mark size=1.5,mark options={fill=vintageorange},
ultra thick,draw=vintageorange,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  01.26  01.26\%
2  01.27  01.27\%
3  01.24  01.24\%
4  11.16  11.16\%
5  59.90  59.90\%
6  80.32  80.32\%
};

\addplot[mark=*,mark size=1.5,mark options={fill=vintagegreen},
ultra thick,draw=vintagegreen,point meta = explicit symbolic]
table[x=x,y=y] {
x y
1  00.60  00.60\%
2  03.89  03.89\%
3  08.89  08.89\%
4  08.25  08.25\%
5  64.97  64.97\%
6  88.86  88.86\%
};
\addlegendentry{\mnist}
\addlegendentry{\yelp}
\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{Max Entropy Classifier (ME)}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[timesaving,
xmax=7.5,
xtick={1, 2, 3, 4, 5, 6, 7},
% xticklabels={0.10, 0.05, 0.01, 5e-3, 1e-3, 5e-4, 1e-4},
xticklabels={0.90, 0.95, 0.99, 0.995, 0.999, 0.9995, 0.9999},
% xlabel shift=0mm,
xlabel=Requested Accuracy ($1-\varepsilon$),
]

\addplot[mark=*,mark size=1.5,mark options={fill=vintageorange},
ultra thick,draw=vintageorange,point meta = explicit symbolic]
table[x=x,y=y,meta=z] {
x y z
1  0.35  0.35\%
2  0.31  0.31\%
3  0.31  0.31\%
4  0.32  0.32\%
5  0.38  0.38\%
6  0.57  0.57\%
7  1.17  1.17\%
};

\addplot[mark=*,mark size=1.5,mark options={fill=vintagegreen},
ultra thick,draw=vintagegreen,point meta = explicit symbolic]
table[x=x,y=y] {
x y
1  4.53  4.53\%
2  4.03  4.03\%
3  3.72  3.72\%
4  3.97  3.97\%
5  5.80  5.80\%
6  8.02  8.02\%
7  29.7  29.7\%
};
\addlegendentry{\higgs}
\addlegendentry{\mnist}
\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{Probabilistic PCA (PPCA)}
\end{subfigure}

\vspace{-2mm}
\caption{\system's relative training time in comparison to full model training. The actual accuracies of the trained models are separately studied in \cref{fig:exp:acc}. The raw data of this figure are in \cref{tab:exp:time_saving}.}
\label{fig:exp:time_saving}
% \vspace{2mm}
\end{figure*}


==> figures/tab_glm.tex <==
\begin{table}[t]
\caption{Examples of Generalized Linear Model.}

\centering
\small
\begin{tabular}{p{20mm} p{30mm} l}
\toprule
\textbf{Exponential}\newline \textbf{family}\newline \textbf{distribution} &
 \textbf{Response}\newline \textbf{function} ($\sigma(\eta)$) &
 \textbf{Model name} \\ \midrule
Gaussian & identity & Linear regression \\
Binomial & logistic (sigmoid) & Logistic regression \\
Multinomial & softmax  &  Softmax regression \\
Gamma & inverse &  \\
Poisson & exponential & \\
\bottomrule
\end{tabular}

\vspace{2mm}

\end{table}

==> figures/tab_models.tex <==

\begin{table}[t]
\caption{Currently available ML models in \system.}
\label{tab:model_classes}

\centering
\small
\begin{tabular}{ll}
\toprule
\textbf{Model Class}  & \textbf{\system Class Name} \\
\midrule
Linear regression      & \texttt{LinearRegression}   \\
Logistic regression    & \texttt{LogisticRegression} \\
Max entropy classifier & \texttt{MaxEntropy}             \\
PPCA                   & \texttt{PPCA}               \\
\bottomrule
\end{tabular}
\end{table}

==> figures/training_time.tex <==
\begin{figure}[t]
  \pgfplotsset{subsampling/.style={
    % width=47mm,
    % height=35mm,
    % ymax=1.4,
    % ymin=0.6,
    x post scale=0.8,
    y post scale=0.8,
    % xmin=1,
    % xmax=6,
    % ylabel=Standard Deviation,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    % xtick={1,2,3,4,5,6,7,8},
    % xticklabels={t1,t9,t12,t15,t17,c1,c2,c3},
    % ytick={0, 50, 100},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    % ylabel shift=-3pt,
    % xlabel shift=-2pt,
    legend style={
        at={(0,1.04)},
        anchor=south west,%column sep=2pt,
        scale=0.8,
        draw=black,fill=none,line width=.5pt,
        % /tikz/every even column/.append style={column sep=40pt}
    },
    % legend style={
    %   at={(0, 1)},
    %   anchor=north west,
    %   fill=none,
    %   scale=0.8,
    % },
    legend columns=2,
    % every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\tiny}
  }}

  \begin{tikzpicture}
    \begin{axis}[subsampling,
      xtick={1, 2, ..., 7},
      xticklabels={1\%,2\%,5\%,10\%,20\%,50\%,100\%,},
      xlabel=Sampling Ratio,
      ylabel=Training Time(s),
      ymode=log,
      colormap/cool,
    ]
      %Below the red parabola is defined
      \addplot[color=myblue,mark=*,mark size=1.5]
      coordinates {
        (1,15.8439) (2,33.0038) (3,70.7212) (4,133.3005) (5,256.2614) (6,638.6638) (7,1316.9)
      };
      \addlegendentry{Logistic Regression}
      \addplot[color=myred,mark=+,mark size=1.5]
      coordinates{
        (1,1460.89) (2,2735.26) (3,6159.38) (4,12551.74) (5,24870.71) (6,63241.35) (7,1316.9)
      };
      \addlegendentry{Bootstrap Logistic}

      %Here the blue parabloa is defined
      \addplot[color=mygreen,mark=square,mark size=1.5]
      coordinates{
        (1,0.4467) (2,0.8081) (3,2.1365) (4,4.0806) (5,8.1725) (6,23.7980) (7,40.9969)
      };
      \addlegendentry{Linear Regression}
      \addplot[color=myyellow,mark=triangle,mark size=1.5]
      coordinates{
        (1,114.7) (2,226.5) (3,644.0) (4,1390.0) (5,2989.2) (6,8424.4) (7,40.9969)
      };
      \addlegendentry{Bootstrap Linear}
    \end{axis}
  \end{tikzpicture}
  \caption{Training Time with Different Sampling Ratios}
  \label{fig:training_time}
\end{figure}

==> mcs.tex <==
\section{Model Class Specification}


==> statistics_computation.tex <==
\section{Computing Necessary Statistics}
\label{sec:hessian}

In this section, we present several methods for computing $H$ (which appears in \cref{thm:param_dist}) and discuss pros and cons of those methods. We also empirically study those methods.

\subsection{Methods}

Computing $J$ is straightforward given $H$ since $J = H - J_r$, where $J_r$ is the Jacobian of $r(\theta)$. We present three methods: (1) ClosedForm, (2) InverseGradients, and (3) ObservedFisher.

\ph{Method 1: ClosedForm}
ClosedForm uses the analytic form of the Jacobian $H(\theta)$ of $g_n(\theta)$, and sets $\theta = \theta_n$ by the definition of $H$. For instance, $H(\theta)$ of L2-regularized logistic regression is expressed as follows:
\[
H(\theta) = \frac{1}{n} X^\top Q X + \beta I
\]
where $X$ is an $n$-by-$d$ matrix whose $i$-th row is $\xx_i$, and $Q$ is a $d$-by-$d$ diagonal matrix whose $i$-th diagonal entry is $\sigma(\theta^\top \xx_i) (1 - \sigma(\theta^\top \xx_i))$, and $\beta$ is the coefficient of L2 regularization. When $H(\theta)$ is available, as in the case of logistic regression, ClosedForm is fast and exact.

However, inverting $H$ is computationally expensive when $d$ is large. Also, using ClosedForm is less straightforward when obtaining analytic expression of $H(\theta)$ is non-trivial. Thus, \system supports ClosedForm only for linear regression and logistic regression. For other methods, such as max entropy classifier and PPCA, either of the following two methods is used.


\ph{Method 2: InverseGradients}
InverseGradients numerically computes $H$ by relying on the Taylor expansion of $g_n(\theta)$: $g_n(\theta_n + d\theta) \approx g_n(\theta_n) + H d\theta$. Since $g_n(\theta_n) = \bm{0}$, the Taylor expansion simplifies to:
\[
g_n(\theta_n + d\theta) \approx H d\theta
\]
The values of $g_n(\theta_n + d\theta)$ and $g_n(\theta_n)$ are computed using the \texttt{grads} function provided by the \mcs. The remaining question is what values of $d\theta$ to use for computing $H$. Since $H$ is a $d$-by-$d$ matrix, \system uses $d$ number of linearly independent $d\theta$ to fully construct $H$. That is, let $P$ be $\epsilon I$, where $\epsilon$ is a small real number ($10^{\minus6}$ by default). Also, let $R$ be the $d$-by-$d$ matrix whose $i$-th column is $g_n(\theta_n + P_{\cdot,i})$ where $P_{\cdot,i}$ is the $i$-th column of $P$. Then,
\[
R \approx H P
\quad \Rightarrow \quad
H \approx R P^{\minus1}
\]
Since InverseGradients only relies on the \texttt{\textbf{grads}} function, it is applicable to all supported models. Although InverseGradients is accurate, it is still computationally inefficient for high-dimensional data, since the \texttt{\textbf{grads}} function must be called $d$ times. We study its runtime overhead in \cref{sec:exp:hessian}.

\ph{Method 3: ObservedFisher}
ObservedFisher numerically computes $H$ by relying on the information matrix equality \cite{efron1978assessing}. According to the information matrix equality, the covariance matrix $C$ of $q(\theta_n; \xx_i, y_i)$ for $i = 1, \ldots, n$ is equal to $J$; then, $H$ can simply be computed as $H = J + J_r$. Instead of computing $C$ directly, however, ObservedFisher takes a slightly different approach to ensure the positive definiteness of $J$ and $H$. This process also ensures the positive definiteness of $H^{\minus1} J H^{\minus1}$, which is the requirement for the covariance matrix of a normal distribution.
Let $Q$ be the $n$-by-$d$ matrix whose $i$-th row is $q(\theta_n; \xx_i, y_i)$. Then, ObservedFisher performs the singular value decomposition of $Q^\top$ to obtain $U$, $\Sigma$, and $V$ such that $Q^\top = U \Sigma V^\top$. Then, ObservedFisher computes $J$ as follows:
\begin{equation}
J = C = Q^\top Q = U\, \Sigma^2\, U^\top \approx U\, \Sigma_+^2\, U^\top
\label{eq:jacobian}
\end{equation}
where $\Sigma_+$ is a diagonal matrix with only positive singular values. Note that the diagonal entries of $\Sigma_+^2$ are the eigenvalues of $J$; because they are also all positive, $J$ is positive definite.

ObservedFisher requires only a single call of the \texttt{\textbf{grads}} function; thus, ObservedFisher is faster than InverseGradients, particularly for high-dimensional data (see \cref{sec:exp:hessian} for experiments). Also, ObservedFisher exposes $U$ and $\Sigma_+$, which are used for \system's custom sampler (\cref{sec:sample}). Due to these reasons, ObservedFisher is \system's default approach to computing $H$ and $J$.


\input{exp_statistics}
